Criticality-Aware RAN Function Placement for Robust 6G Networks

The disaggregation of base stations into radio access network (RAN) functions introduces new vulnerabilities to mobile networks, as disruptions in cloud locations can interrupt multiple RAN functions and trigger cascading failures, leading to widespread outages. In this paper, we propose a criticality-aware RAN function placement solution to improve the robustness of disaggregated mobile networks against random failures and targeted attacks. Our solution optimizes the placement of centralized units (CUs) and distributed units (DUs) across cloud locations to reduce functional dependencies and limit the criticality of cloud locations, while preserving the cost benefits of RAN function centralization. We formulate the placement as an optimization model that jointly minimizes functional dependency and placement cost, subject to criticality constraints, as well as computing and transport requirements. We numerically evaluated our approach on a real-world mobile network topology across multiple disruption scenarios and demonstrated that our solution improves robustness, yielding up to 75% more operational radio units (RUs) after disruptions than existing approaches.

==> Tables/splits.tex <==
\begin{table}[h]
\footnotesize
\centering
\begin{tabular}{c|cccc}
\hline
\textbf{Option} & \textbf{\begin{tabular}[c]{@{}c@{}}Functional\\ Split\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}One-way\\ Latency\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Bitrate (Gbps)\\ Downlink\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}CPU \\ (cores)\end{tabular}} \\ \hline
O1              & RRC -- PDCP                                                          & 10 ms                                                              & 4                                                                          & 0.49                   \\
O2              & PDCP -- H-RLC                                                        & 10 ms                                                              & 4                                                                          & 0.49                   \\
O3              & H-RLC -- L-RLC                                                       & 10 ms                                                              & 4                                                                          & 0.0245                 \\
O4              & L-RLC -- H-MAC                                                       & 1 ms                                                               & 4                                                                          & 0.0245                 \\
O5              & H-MAC -- L-MAC                                                       & $ < 1 ms$                                                          & 4                                                                          & 0.343                  \\
O6              & L-MAC -- H-PHY                                                       & 250 $\mu$s                                                         & 4.13                                                                       & 0.343                  \\
O7              & H-PHY -- L-PHY                                                       & 250 $\mu$s                                                         & 86.1                                                                       & 0.833                  \\
O8              & L-PHY -- RF                                                          & 250 $\mu$s                                                         & 157.3                                                                      & 2.352    \\ \hline             
\end{tabular}
\caption{Functional split options and demands.}
\label{tab:functional_splits}
\end{table}

==> tmp/tables/mdc.tex <==


\definecolor{babyblueeyes}{rgb}{0.63, 0.79, 0.95}
\definecolor{bluegray}{rgb}{0.4, 0.6, 0.8}
\definecolor{header}{rgb}{0.9, 0.9, 0.9}
\definecolor{lines}{rgb}{0.6, 0.6, 0.6}


\newcommand{\thead}[1]{\multicolumn{1}{|c|}{\bfseries #1}}

\newcommand{\csize}{0.8\columnwidth}
\begin{table}[!ht]
\caption{\acp{MDC}' specifications}
\label{tab:mdc}


\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\thead{\ac{MDC}} & \thead{Processor} &  \thead{$\vm$} & \thead{$\procsmdc_{\vm\mdc}$} &\thead{$\coresproc_{\vm\mdc}$} & \thead{$\clockproc_{\vm\mdc}$} &  \thead{$\priceproc_{\vm\mdc}$} \\ \hline


\multirow{2}{*}{Macrocell} & D-1653 & 1 & 11 & 8 & 2.8 $GHz$ & 0.340 \\ \cline{2-7}
  & D-1667 & 2 & 11 & 12 & 2.7 GHz & 0.510\\ \hline
\multirow{2}{*}{Smallcell} & D-1513N & 3 & 7 & 4 & 2.2 GHz & 0.170 \\ \cline{2-7}
 & D-1633N & 4 & 7 & 6 & 2.5 GHz & 0.255 \\ \hline
 

\end{tabular}
\end{table}

==> tmp/utils/acronym.tex <==
\begin{acronym}
  \acro{H-CRAN} {Heterogeneous Cloud Radio Access Network}
  \acro{HetNet} {Heterogeneous Network}
  \acro{C-RAN} {Cloud Radio Access Network}
  \acro{RRH} {Remote Radio Head}
  \acro{BBU} {Base-Band Unit}
  \acro{vBBU} {virtual Base-Band Unit}
  \acro{FEC} {Forward Error Correction}
  \acro{HARQ} {Hybrid Automatic Repeat reQuest}
  \acro{LTE-A} {Long Term Evolution Advanced}
  \acro{LTE} {Long Term Evolution}
  \acro{RAN} {Radio Access Network}
  \acro{BER} {Bit Error Rate}
  \acro{Eb/No} {Energy per bit to noise power spectral density ratio}
  \acro{ms} {millisecond}
  \acro{BS} {Base Station}
  \acro{UE} {User Equipment}
  \acro{SNR} {Signal-to-Noise ratio}
  \acro{RAT} {Radio Access Technologies}
  \acro{QoS} {Quality of Service}
  \acro{QoE} {Quality of Experience}
  \acro{GPP} {General Purpose Processor}
  \acro{D2D} {Device-to-Device communication}
  \acro{WiFi} {Wireless Fidelity}
  \acro{F-RAN}{Fog Radio Access Networks}
  \acro{MDC}{Micro Data Center}
  \acro{DC}{Data Center}
  \acro{eICIC}{enhanced Inter-Cell Interference Control}
  \acro{SDN}{Software-Defined Networking}
  \acro{SDWN}{Software-Defined Wireless Networking}
  \acro{km}{Kilometer}
  \acro{CP}{Central Processor}
  \acro{HSPA}{High Speed Packet Access}
  \acro{JT}{Joint Transmission}
  \acro{AWGN}{Additive White Gaussian Noise}
  \acro{Hz}{hertz}
  \acro{QAM}{Quadrature Amplitude Modulation}
  \acro{MIMO}{Multiple-Input Multiple-Output}
  \acro{F-RAN}{Fog Radio Access Network}
  \acro{AI}{Artificial Intelligence}
  \acro{DRL}{Deep Reinforcement Learning}
  \acro{MAS}{Multi-agent System}
  \acro{MCS}{Modulation and Coding Scheme}
  \acro{KB}{Knowledge Base}
  \acro{ASP}{Application Service Provider}
  \acro{CQI}{Channel Quality Indicator}
  \acro{CPU}{Central Processing Unit}
  \acro{FIPA}{Foundation for Intelligent Physical Agents}
  \acro{ACL}{Agent Communication Language}
  \acro{VM}{Virtual Machine}
  \acro{BILP}{Binary Integer Linear Programming}
  \acro{mbps}{Megabit per second}
  \acro{bps}{Bits per second}
  \acro{CDR}{Call Detail Record}
  \acro{3GPP}{Third Generation Partnership Project}
\end{acronym}




==> tmp/utils/preamble.tex <==
%*************************************************************
%*****    PREAMBLE
%*************************************************************

%!TEX TS-program =  pdflatex

%*************************************************************
%*****    PACKAGES
%*************************************************************
\usepackage{chapterbib}
\usepackage[english]{babel}
\usepackage{graphicx,url}       % pacote para importar figuras
\usepackage{mathptmx}           % p/ usar fonte Adobe Times
\usepackage{epsfig}
\usepackage{subfigure}
\usepackage[dvipsnames,svgnames,table]{xcolor}
\usepackage{hhline}
\usepackage{etoolbox}
\usepackage{cellspace}
\setlength\cellspacetoplimit{4pt} 
\setlength\cellspacebottomlimit{4pt}
% \usepackage[table]{xcolor}
\usepackage{subfigure}
% \usepackage{times}              % pacote para usar fonte Adobe Times

%\usepackage{subcaption}

\usepackage{pdfpages}
% \usepackage{natbib} 
% \usepackage{bibentry} 
\usepackage{url}
\usepackage{color}
\usepackage{xspace}

\usepackage{listings}
\usepackage{tabularx}
\usepackage{array}
% \usepackage{caption}
% \usepackage{subcaption}
\usepackage{pbox}
\newcommand{\tabitem}{~~\llap{\textbullet}~~}

\usepackage{multirow} 
\hyphenation{ma-shu-ps m-b-d-s-a-s}
\newcommand{\tabitemm}{~~\llap{\textbullet}~~}
% \usepackage{setspace}
% \setstretch{0.955}
%----------------------------------------------------------------------
%% AMS group
%----------------------------------------------------------------------
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{amsthm}

%----------------------------------------------------------------------
%% Fonts and alphabets (beware of conflicts)
%----------------------------------------------------------------------
% \usepackage[utf8]{inputenc}
\usepackage[latin1]{inputenc}   % Brazilian accentuation support
\usepackage[T1]{fontenc}
\usepackage{algpseudocode,algorithm,algorithmicx}
% \usepackage{algorithmic}
% \usepackage[plain]{algorithm}
%% Minion Pro
%----------------------------------------------------------------------
%\linespread{1.05}
%\usepackage[lf,minionint,openg,footnotefigures]{MinionPro}
%\usepackage[bib,eqno,enum]{tabfigures}
%\input glyphtounicode
%\pdfgentounicode=1

%% Libertine 
%----------------------------------------------------------------------
%\usepackage[proportional,lining]{libertine}
%\usepackage[libertine,libaltvw,cmintegrals]{newtxmath}

%% Garamond
%----------------------------------------------------------------------
%\usepackage[full]{textcomp}
%\usepackage{garamondx}
%\usepackage[garamondx,cmintegrals,cmbraces]{newtxmath}
%\useosf

%\usepackage[urw-garamond]{mathdesign}
%\usepackage{garamondx}

%% Charter
%----------------------------------------------------------------------
%\usepackage[bitstream-charter]{mathdesign}

%% Palatino (uncomment one, not both)
%----------------------------------------------------------------------
% \linespread{1.05}
%\usepackage{newpxtext,newpxmath}
% \usepackage[sc]{mathpazo}

%% Times
%----------------------------------------------------------------------
%\usepackage{txfonts}

%% Sans serif font (biolinum)
%----------------------------------------------------------------------
%\usepackage[sf]{libertine}

%% Typewriter font (inconsolata)
%----------------------------------------------------------------------
%\usepackage[varqu,varl]{zi4}


%% Math alphabets
%----------------------------------------------------------------------
% \usepackage[mathcal]{euscript}
%\usepackage[%
%cal=euler,
%%scr=euler,
%frak=euler
%]
%{mathalfa}


%----------------------------------------------------------------------
%% Colors
%----------------------------------------------------------------------
\definecolor{MyBlue}{HTML}{5f8dd3}
\newcommand{\green}[1]{\textcolor{ForestGreen}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\magenta}[1]{\textcolor{magenta}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\definecolor{lightgray}{gray}{0.9}
\definecolor{darkgray}{gray}{0.5}
%----------------------------------------------------------------------
%% Figures and Graphics
%----------------------------------------------------------------------
%\usepackage{float}
%\usepackage{subfigure}
%\usepackage{tikz}


%----------------------------------------------------------------------
%% Miscellaneous
%----------------------------------------------------------------------
% \usepackage{acronym}
\usepackage[nolist,nohyperlinks]{acronym}
% \usepackage[acronym,toc]{glossaries}
% \usepackage[nohyperlinks]{acronym}
%\usepackage{bbold}
%\usepackage{latexsym}
%\usepackage{paralist}
%\usepackage{wasysym}
% \usepackage{xspace}


%----------------------------------------------------------------------
%% References
%----------------------------------------------------------------------
% \usepackage[numbers,sort&compress]{natbib}
% \def\bibfont{\footnotesize}
% \def\bibsep{\smallskipamount}
% \def\bibhang{24pt}


%----------------------------------------------------------------------
%% Hyperlinks
%----------------------------------------------------------------------
% \usepackage{hyperref}
% \hypersetup{
%   draft=false,
%   colorlinks=true,
%   linktocpage=true,
%   %pdfstartpage=1,
%   pdfstartview=FitH,
%   breaklinks=true,
%   pdfpagemode=UseNone,
%   pageanchor=true,
%   pdfpagemode=UseOutlines,
%   plainpages=false,
%   bookmarksnumbered,
%   bookmarksopen=false,
%   bookmarksopenlevel=1,
%   hypertexnames=true,
%   pdfhighlight=/O,
%   %hyperfootnotes=true,
%   %nesting=true,
%   %frenchlinks,
%   urlcolor=Maroon,linkcolor=MyBlue,citecolor=DarkGreen, % <--- for screen
%   %urlcolor=black, linkcolor=black, citecolor=black, %pagecolor=black, % <--- for printing
%   %pagecolor=RoyalBlue,
%   pdftitle={},
%   pdfauthor={},
%   pdfsubject={},
%   pdfkeywords={},
%   pdfcreator={pdfLaTeX},
%   pdfproducer={LaTeX with hyperref}
% }

% Hyperlink shortcuts
\def\EMAIL#1{\href{mailto:#1}{#1}}
\def\URL#1{\href{#1}{#1}}


%----------------------------------------------------------------------
%% Backrefs
%----------------------------------------------------------------------
%\newcommand{\backrefnotcitedstring}{\relax} %(Not cited.)
%\newcommand{\backrefcitedsinglestring}[1]{(Cited on page~#1.)}
%\newcommand{\backrefcitedmultistring}[1]{(Cited on pages~#1.)}

%\RequirePackage[hyperpageref]{backref} % to be loaded after hyperref package 
%   \renewcommand{\backreftwosep}{ and~} % seperate 2 pages
%   \renewcommand{\backreflastsep}{, and~} % seperate last of longer list
%   \renewcommand*{\backref}[1]{} % Disable standard
%   \renewcommand*{\backrefalt}[4]{ % Detailed backref
%      \ifcase #1 %
%         \backrefnotcitedstring %
%      \or
%         \backrefcitedsinglestring{#2} %
%      \else
%         \backrefcitedmultistring{#2} %
%      \fi}



%*************************************************************
%*****    MACROS
%*************************************************************

%----------------------------------------------------------------------
%% Bold Symbols
%----------------------------------------------------------------------
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}

\newcommand{\ba}{\mathbf{a}}
\newcommand{\bolddb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\boldd}{\mathbf{d}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\boldf}{\mathbf{f}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bi}{\mathbf{i}}
\newcommand{\bj}{\mathbf{y}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bl}{\mathbf{l}}
\newcommand{\bm}{\mathbf{m}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}

%----------------------------------- %

%----------------------------------------------------------------------
%% Fields
%----------------------------------------------------------------------
\newcommand{\F}{\mathbb{F}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}


%----------------------------------------------------------------------
%% Operators
%----------------------------------------------------------------------
\DeclareMathOperator{\argdot}{\cdotp}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\bd}{bd}
\DeclareMathOperator{\bigoh}{\mathcal O}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\cl}{cl}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\diver}{div}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\eig}{eig}
\DeclareMathOperator{\ess}{ess}
\DeclareMathOperator{\ex}{\mathbb{E}}
%\DeclareMathOperator{\exclude}{\setminus}
\DeclareMathOperator{\expit}{expit}
\DeclareMathOperator{\grad}{\nabla}
\DeclareMathOperator{\logit}{logit}
\DeclareMathOperator{\hess}{Hess}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\ind}{ind}
\DeclareMathOperator{\intr}{int}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\midd}{\|}
\DeclareMathOperator{\one}{\mathbb{1}}
\DeclareMathOperator{\pr}{pr}
\DeclareMathOperator{\prob}{\mathbb{P}}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\rel}{rel}
\DeclareMathOperator{\relint}{rel\,int}
\DeclareMathOperator{\sign}{sgn}
%\DeclareMathOperator{\simplex}{\Delta}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\var}{Var}
\DeclareMathOperator{\vol}{Vol}

\DeclareMathOperator*{\intersect}{\bigcap}
\DeclareMathOperator*{\lip}{lip}
\DeclareMathOperator*{\union}{\bigcup}


%----------------------------------------------------------------------
%% Shorthands
%----------------------------------------------------------------------
\newcommand{\dd}{\:d}
\newcommand{\del}{\partial}
\newcommand{\eps}{\varepsilon}
\newcommand{\exclude}[1]{\operatorname\setminus\left\{#1\right\}}
\newcommand{\from}{\colon}
\newcommand{\injects}{\hookrightarrow}
\newcommand{\iq}{\mathrm{i}}
\newcommand{\mg}{\succ}
\newcommand{\mgeq}{\succcurlyeq}
\newcommand{\ml}{\prec}
\newcommand{\mleq}{\preccurlyeq}
\newcommand{\pd}{\partial}
\newcommand{\simplex}{\Delta}
\newcommand{\intsimplex}{\simplex^{\!\circ}}
\newcommand{\wilde}{\widetilde}


%----------------------------------------------------------------------
%% Delimiters
%----------------------------------------------------------------------
\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\bra}[1]{\left\langle #1 \right\vert}
\newcommand{\ket}[1]{\left\vert #1 \right\rangle}
\newcommand{\braket}[2]{\left\langle #1 \middle\vert  #2 \right\rangle}
\newcommand{\product}[2]{\left\langle #1,  #2 \right\rangle}


%----------------------------------------------------------------------
%% Math display and formatting
%----------------------------------------------------------------------
\newcommand{\dis}{\displaystyle}
\newcommand{\txs}{\textstyle}

\newcommand{\insum}{\sum\nolimits}
\newcommand{\inprod}{\prod\nolimits}
\newcommand{\mb}{\mathbf}




%*************************************************************
%*****    EDITING
%*************************************************************
\usepackage[textwidth=30mm]{todonotes}
%\setlength{\marginparwidth}{2cm}
\usepackage{soul}
\usepackage{setspace}
\setstretch{0.9707}
\setstcolor{red}
\sethlcolor{SkyBlue}

\newcommand{\needref}{{\color{red} \upshape [\textbf{??}]}\xspace}
\newcommand{\attn}{{\color{red} \upshape [\textbf{!!}]}\xspace}




%*************************************************************
%*****    ENVIRONMENTS
%*************************************************************

%----------------------------------------------------------------------
%% Theorem-like
%----------------------------------------------------------------------
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem*{corollary*}{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}

%----------------------------------------------------------------------
%% Definition-like
%----------------------------------------------------------------------
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem*{definition*}{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{objective}[theorem]{Objective}

%----------------------------------------------------------------------
%% Remark-like
%----------------------------------------------------------------------
\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem{example}{Example}

%----------------------------------------------------------------------
%% Numbering
%----------------------------------------------------------------------
%\numberwithin{equation}{section}
%\numberwithin{theorem}{section}
%\numberwithin{remark}{section}
%\numberwithin{example}{section}




%*************************************************************
%*****    PAPER-SPECIFIC STUFF
%*************************************************************

%----------------------------------------------------------------------
% Sets
%----------------------------------------------------------------------
% I (VMs)
\newcommand{\vm}{i}
\newcommand{\vms}{\mathrm{I}}
\newcommand{\vmset}{\mathcal{I}}

\newcommand{\vmmc}{j}
\newcommand{\vmsmc}{\mathrm{J}}
\newcommand{\vmsetmc}{\mathcal{J}}

\newcommand{\vmsc}{j'}
\newcommand{\vmssc}{\mathrm{J'}}
\newcommand{\vmsetsc}{\mathcal{J'}}

% S (MDCs)
% Macro
\newcommand{\mdcmc}{u}
\newcommand{\mdcsmc}{\mathrm{U}}
\newcommand{\mdcsetmc}{\mathcal{U}}
% Small
\newcommand{\mdcsc}{u'}
\newcommand{\mdcssc}{\mathrm{U'}}
\newcommand{\mdcsetsc}{\mathcal{U'}}
% Total (U U U')
\newcommand{\mdc}{s}
\newcommand{\mdcs}{\mathrm{S}}
\newcommand{\mdcset}{\mathcal{S}}

% M (RRHs)
% Macro 
\newcommand{\rrhmc}{v}
\newcommand{\rrhsmc}{\mathrm{V}}
\newcommand{\rrhsetmc}{\mathcal{V}}
% Small
\newcommand{\rrhsc}{v'}
\newcommand{\rrhssc}{\mathrm{V'}}
\newcommand{\rrhsetsc}{\mathcal{V'}}
% Total (V U V')
\newcommand{\rrh}{m}
\newcommand{\rrhs}{\mathrm{M}}
\newcommand{\rrhset}{\mathcal{M}}

% T
\newcommand{\slot}{t}
\newcommand{\slots}{\mathrm{T}}
\newcommand{\slotset}{\mathcal{T}}


% Composite values / Parameters
% VMs
\newcommand{\minvms}{n} % minimum number of VMs

\newcommand{\clockproc}{f} % processor's clock (GHz)
\newcommand{\effproc}{e} % processor's efficiency (instructions per cycle)
\newcommand{\coresproc}{p} % number of cores per processor 
\newcommand{\priceproc}{k} % cost per VM (USD)

% Misc
\newcommand{\procsmdc}{g} % processors per mdc

\newcommand{\pricelease}{k_{lease}} % processors per mdc

\newcommand{\workload}{\Gamma} % Workload per RRH per slot t (Gamma_mt) (mbps)

\newcommand{\decoding}{w} % channel decoding (number of instructions)
\newcommand{\dmacromacro}{d_{macro}} % distance between macro (m)

\newcommand{\delaybudget}{\varphi} % delay budget (s)

\newcommand{\hops}{h} % d_hops (m)
\newcommand{\delayhop}{\lambda} % delay per hop (s)
\newcommand{\distance}{d} % d_sm (distance between mdc-rrh)
\newcommand{\lightspeed}{c} % light speed (m/s)


\newcommand{\totalcores}{A_{cores}}
\newcommand{\idlecores}{U_{cores}}
\newcommand{\totalcost}{K_{alloc}}
\newcommand{\maxincome}{G_{lease}}



%Binary variables
\newcommand{\avmmdcrrh}{a}



%----------------------------------------------------------------------
%% Sundries
%----------------------------------------------------------------------




%*************************************************************
%*****    AUTHOR-SPECIFIC COMMANDS
%*************************************************************

\newcommand{\negspace}{\!\!\!}
\newcommand{\refeq}[1]{(\ref{#1})}   
\newcommand{\reffig}[1]{Fig.~\ref{#1}}
\newcommand{\reftable}[1]{Table~\ref{#1}}  



\newcommand{\ie}{\textit{i.e., }}                   %i.e.,
\newcommand{\eg}{\textit{e.g., }}                   %e.g., 
\newcommand{\etal}{\textit{et al. }}               %Et al.
\newcommand{\facto}{\textit{, the facto, }}         %, the facto, 

\newcommand{\node}{\eta}
\newcommand{\edge}{\varepsilon}
\newcommand{\func}{G($\node,\edge$)}

\newcommand{\1}{(\textit{i})}
\newcommand{\2}{(\textit{ii})}
\newcommand{\3}{(\textit{iii})}
\newcommand{\4}{(\textit{iv})}
\newcommand{\A}{(\textit{a}) }
\newcommand{\B}{(\textit{b}) }

\newcommand{\fognode}{Fog-\ac{RRH}\xspace}
\newcommand{\fognodes}{Fog-\acp{RRH}\xspace}
\newcommand{\minsec}{minutes/seconds\xspace}


